Large Language Models Are Reasoning Teachers

Recent works have shown that chain-of-thought (CoT) prompting can elicit language models to solve complex reasoning tasks, step-by-step. However, prompt-based CoT methods are dependent on very large models such as GPT-3 175B which are prohibitive to deploy at scale. In this paper, we use these large models as reasoning teachers to enable complex reasoning in smaller models and reduce model size requirements by several orders of magnitude. We propose Fine-tune-CoT, a method that generates reasoning samples from very large teacher models to fine-tune smaller models. We evaluate our method on a wide range of public models and complex tasks. We find that Fine-tune-CoT enables substantial reasoning capability in small models, far outperforming prompt-based baselines and even the teacher model in many tasks. Additionally, we extend our method by leveraging the teacher model's ability to generate multiple distinct rationales for each original sample. Enriching the fine-tuning data with such diverse reasoning results in a substantial performance boost across datasets, even for very small models. We conduct ablations and sample studies to understand the emergence of reasoning capabilities of student models. Our code implementation and data are available at https://github.com/itsnamgyu/reasoning-teacher.

==> old.tex <==
% Old main figure on data scalability
% \begin{figure}[t]
%     \centering
%     \resizebox{\linewidth}{!}{
%         \includegraphics{figures/scalability_multiarith.pdf}
%     }
%     \caption{
%     \textbf{Fine-tune-CoT elicits reasoning capabilities in small LMs}.
%     Accuracy is reported for student models (GPT-3 6.7B) on the MultiArith dataset.
%     ``Fine-tune'' refers to standard fine-tuning on the full dataset, and ``Zero-shot-CoT'' refers to the recent prompt-based reasoning method by \citet{kojima2022large}.
%     Zero-shot-CoT is used for the teacher (GPT-3 175B) to generate reasoning to teach students, but is ineffective when directly applied to smaller models.
%     Fine-tune-CoT performance is highly scalable with data, while standard fine-tuning and prompt-based methods both have limited data scalability (Section XXX).
%     }
%     \label{fig:scalability}
% \end{figure}

%1111111111111111111111111111111111111111
%2222222222222222222222222222222222222222
%3333333333333333333333333333333333333333

% Few-shot Fine-tune-CoT for 6.7B >> replaced by full performance table in Appendix.
% \begin{table}[t]
% \begin{minipage}[b]{1.0\linewidth}
% \caption{
%     Accuracy (\%) of baseline Zero-shot-CoT and Fine-tune-CoT methods as well as Fine-tune-CoT using {8, 32, 128}-shot fine-tuning data.
%     Results are reported for the GPT-3 6.7B model.
% }
% \label{tab:few_shot}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llllll}
% \toprule
%  & Zero-shot-CoT & \multicolumn{4}{l}{Fine-tune-CoT} \\
%  &  & 8-shot & 32-shot & 128-shot & Full \\
% \midrule
% SingleEq & 1.32 & 5.26 & 8.55 & 13.82 & 21.05 \\
% AddSub & 2.52 & 12.61 & 18.49 & 22.69 & 20.17 \\
% MultiArith & 5.00 & 0.56 & 12.22 & 17.78 & 34.44 \\
% GSM8K & 2.35 & 0.83 & 2.43 & 2.65 & 7.20 \\
% AQUA & 21.26 & 11.81 & 9.45 & 12.60 & 16.93 \\
% SVAMP & 1.33 & 2.00 & 8.00 & 7.33 & 12.67 \\
% \midrule
% CommonSenseQA & 19.98 & 13.84 & 19.41 & 22.60 & 51.27 \\
% StrategyQA & 51.09 & 31.73 & 40.47 & 43.81 & 47.16 \\
% \midrule
% Date Understanding & 15.32 & 0.90 & 18.02 & 26.13 & 60.36 \\
% Coin Flip (4 words) & 46.67 & 45.33 & 100.00 & 98.67 & 98.00 \\
% Shuffled Objects & 31.11 & 28.44 & 34.22 & 47.56 & 64.00 \\
% Last Letter (4 words) & 0.00 & 2.00 & 21.33 & 42.67 & 52.00 \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


